Generating Test Scenarios from NL Requirements using Retrieval-Augmented LLMs: An Industrial Study

Test scenarios are specific instances of test cases that describe actions to validate a particular software functionality. By outlining the conditions under which the software operates and the expected outcomes, test scenarios ensure that the software functionality is tested in an integrated manner. Test scenarios are crucial for systematically testing an application under various conditions, including edge cases, to identify potential issues and guarantee overall performance and reliability. Specifying test scenarios is tedious and requires a deep understanding of software functionality and the underlying domain. It further demands substantial effort and investment from already time- and budget-constrained requirements engineers and testing teams. This paper presents an automated approach (RAGTAG) for test scenario generation using Retrieval-Augmented Generation (RAG) with Large Language Models (LLMs). RAG allows the integration of specific domain knowledge with LLMs' generation capabilities. We evaluate RAGTAG on two industrial projects from Austrian Post with bilingual requirements in German and English. Our results from an interview survey conducted with four experts on five dimensions -- relevance, coverage, correctness, coherence and feasibility, affirm the potential of RAGTAG in automating test scenario generation. Specifically, our results indicate that, despite the difficult task of analyzing bilingual requirements, RAGTAG is able to produce scenarios that are well-aligned with the underlying requirements and provide coverage of different aspects of the intended functionality. The generated scenarios are easily understandable to experts and feasible for testing in the project environment. The overall correctness is deemed satisfactory; however, gaps in capturing exact action sequences and domain nuances remain, underscoring the need for domain expertise when applying LLMs.

==> Files/analysis.tex <==
\subsection{Evaluation Procedure}\label{subsec:analysis} 
We answer our RQs using the experiments below. 


==> Files/camera-ready-notes.tex <==
- remove anonymous authors from bib -- done
- remove the redacted for the doc collection 
- remove ``Amendment details are redacted for
double-blind review.'' and update date and country
- add affiliation - corresponding author
- add acknowledgement
- remove new page from before references 


==> Files/results.tex <==
\section{Results}\label{sec:results}



% \begin{table*}
% %\footnotesize
% \centering
% \caption{Full Page Example TABLE.}
% \label{tab:table_label}
% \begin{threeparttable}[t]
% \begin{tabularx}{0.96\textwidth}{@{} p{0.08\textwidth} @{\hskip 0.5em} p{0.05\textwidth} @{\hskip 0.5em} *{4}{>{\centering\arraybackslash}X}@{}}
%     \toprule
% Domain &  Col1 & Col2 & Col3 & Col4 & Col5 \\ 
% \midrule
% R1 & 1158 & \textbf{100}  & \textbf{100} & 99.0  & \textbf{100}   \\   
% R2 & 781 & \textbf{100}  & \textbf{100} & 98.9  & \textbf{100} \\
% R3 & 50  & \textbf{100} & \textbf{100}   & 91.7 & \textbf{100}\\ 
% \bottomrule
% \end{tabularx}
% \begin{tablenotes}
%      \item[$\dag$] Some notes can be added here (optional). 
%      \end{tablenotes}
%  \end{threeparttable}
%  %\vspace*{-1.2em}
% \end{table*}






